Ablation Study of How Run Time Assurance Impacts the Training and Performance of Reinforcement Learning Agents

Reinforcement Learning (RL) has become an increasingly important research area as the success of machine learning algorithms and methods grows. To combat the safety concerns surrounding the freedom given to RL agents while training, there has been an increase in work concerning Safe Reinforcement Learning (SRL). However, these new and safe methods have been held to less scrutiny than their unsafe counterparts. For instance, comparisons among safe methods often lack fair evaluation across similar initial condition bounds and hyperparameter settings, use poor evaluation metrics, and cherry-pick the best training runs rather than averaging over multiple random seeds. In this work, we conduct an ablation study using evaluation best practices to investigate the impact of run time assurance (RTA), which monitors the system state and intervenes to assure safety, on effective learning. By studying multiple RTA approaches in both on-policy and off-policy RL algorithms, we seek to understand which RTA methods are most effective, whether the agents become dependent on the RTA, and the importance of reward shaping versus safe exploration in RL agent training. Our conclusions shed light on the most promising directions of SRL, and our evaluation methodology lays the groundwork for creating better comparisons in future SRL work.

==> literature_review.tex <==
% \subsubsection{Paper title}
% \textbf{author, conference/journal, year, \href{}{link}}

% \subsection{Category (e.g. RL, reachability, ML, etc)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% (Deep) Reinforcement Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{(Deep) Reinforcement Learning}
This subsection contains papers related to general RL type things. The Safe RL papers will be more focused on what makes those methods "Safe". This is a link for term definitions that I'll need to double check against what I have: \href{https://towardsdatascience.com/the-complete-reinforcement-learning-dictionary-e16230b7d24e}{RL dictionary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A (Long) Peek into Reinforcement Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{A (Long) Peek into Reinforcement Learning (Lil'Log)}
\textbf{Lillian Weng, Lil'Log, 2018, \href{https://lilianweng.github.io/lil-log/2018/02/19/a-long-peek-into-reinforcement-learning.html#key-concepts}{link}}

This blog post, which is highly recommended to people new to RL, explains the concepts of RL in somewhat simpler terms. In essence, this is a summary of a summary.

\textbf{What is RL?}: The goal of RL is to learn a good strategy for an agent to complete a task from experimental trials that have their levels of success represented as a reward. With the optimal strategy, the agent is capable to actively adapt to the environment to maximize future rewards. This is done by an agent choosing actions in an environment. This is illustrated in Figure \todo{get figure describing interaction of agent and environment, probably figure 3 from this blog}

The types of RL are defined by how they use 3 distinct components and combinations of them. These components are:
\begin{itemize}
    \item \textbf{Model}: a descriptor of the environment. With a model, we can learn or infer how the environment responds to different actions. The major components of a model are the transition probability function and a reward function.
    \item \textbf{Policy}: the agent's behavior function, often denoted as $\pi$, is a mapping from state, $s$, to action, $a$, and can be deterministic, $\pi(s)=a$ or stochastic, $\pi(a|s) = P_\pi [A=a|S=s]$.
    \item \textbf{Value Function}: a measure of the "goodness" of a state or how rewarding a state-action pair is based on future rewards. This future reward, or \emph{return}, is a total sum of discounted rewards computed with discount factor $\gamma \in [0,1]$: $G_t = \sum_{k=0}^{\infty} \gamma^k R_{t+k+1}$
    \begin{itemize}
        \item \textbf{state-value}: the expected return if the agent is in state $s$ at time $t$: $V_\pi (s) = E_\pi [G_t |S_t = s]$
        \item \textbf{action-value}: also known as the Q-value is the expected return of a given state-action pair: $Q_\pi (s,a)=E_\pi [G_t |S_t =s,A_t =a]$ This can be used to estimate the state-value using the target policy. $V_\pi =\sum_{a \in A} Q_\pi (s,a)\pi(a|s)$
        \item \textbf{advantage}: the difference between the action-value and the state-value (this is used in A2C-based algorithms). It is defined as: $A_\pi(s,a)=Q_\pi(s,a)-V_\pi(s)$
    \end{itemize}
\end{itemize}
Some key things/terms to know when talking about these components are:
\begin{itemize}
    \item \textbf{Model-based:} Rely on the model of the environment; either the model is known or the algorithm learns it explicitly.
    \item \textbf{Model-free:} No dependency on the model during learning.
    \item \textbf{On-policy:} Use the deterministic outcomes or samples from the target policy to train the algorithm.
    \item \textbf{Off-policy:} Training on a distribution of transitions or episodes produced by a different behavior policy rather than that produced by the target policy.
\end{itemize}

\textbf{Temporal-Difference Learning (TD)}: Model-free learning from episodes of experience. The key thing about TD that makes it so important (“one idea … central and novel to reinforcement learning” \todo{cite Sutton\&Barto}) is that it can learn from \emph{incomplete} episodes. We don't have to track the episode to termination using TD learning. This is because of \emph{Value Estimation}.

\textbf{Value Estimation} is a key idea of Temporal-Difference Learning where the value function, $V(S_t)$, is updated towards an estimated return, or TD target. The updates in the value function are determined by the learning rate, $\alpha$ so that $V(S_t) \gets V(S_t) + \alpha (R_{t+1} + \gamma V(S_{t+1}) - V(S_t))$. The same can be done for the Q-value where $Q(S_t,A_t) \gets Q(S_t,A_t) + \alpha (R_{t+1} + \gamma Q(S_{t+1},A_{t+1}) - Q(S_t,A_t))$. This adaptation for the Q-value led to the creation of algorithms \emph{SARSA} and \emph{Q-Learning}.

\textbf{Q-Learning}, developed by Watkins \& Dayan in 1992, was a major step forward in early RL. It is very similar to \emph{SARSA} except for one key difference in their steps. \emph{SARSA} updates every 2 steps, using what was learned in the second step to evaluate the change for the previous step. \emph{Q-Learning}, on the other hand, uses an estimate of the Q values, $Q_*$ to choose the next action independent of the policy. Thus, \emph{Q-Learning} is also \emph{off-policy}. These are the steps in \emph{Q-Learning}:
\begin{enumerate}
    \item From time step $t$ at state $S_t$, pick an action, $A_t$ according to the Q values, usually in a $\sigma$-greedy approach
    \item With action $A_t$, we observe reward $R_t$ and a transition to state $S_{t+1}$
    \item Update the Q-function according to: $Q(S_t,A_t) \gets Q(S_t,A_t) + \alpha (R_{t+1} + \gamma \max_{a \in A} Q(S_{t+1},a) - Q(S_t,A_t))$
    \item increment $t$ and repeat from step 1
\end{enumerate}

\emph{Q-Learning} has a problem though. Theoretically, the Q values can be saved for every state-action pair, but that quickly becomes infeasible as the state-action space gets larger. Thus, a function can be used to approximate the Q values. The best way to do this is with \textbf{Deep Q-Network}s (\emph{DQN}). In order for \emph{DQN} to work and not suffer from instability and divergence, it requires two mechanisms:
\begin{itemize}
    \item \textbf{Experience Replay}: all the steps in an episode are recorded in replay memory, $D_t$, which has experience tuples over many episodes. During updates, samples from $D_t$ are drawn at random and included in the update process and can be used multiple times. Experience Replay removes correlations in observation sequences and smooths over changes in data distribution.
    \item \textbf{Periodically Updated Target}: Update Q towards target values that are only periodically updated. Every $C$ (hyperparameter) steps, the Q network is cloned and kept frozen as the optimization target. This makes training more stable by overcoming short-term oscillations.
\end{itemize}
The loss function for this looks like: 
\begin{equation*}
    L(\theta) = E_{(s,a,r,s')\sim U(D)}[(r + \gamma \max_{a'}Q(s',a';\theta^-) - Q(s,a;\theta))^2]
\end{equation*} 
where $U(D)$ is a uniform distribution over the replay memory and $\theta^-$ is the frozen target Q-network

Back to on-policy methods, \textbf{Policy Gradient} methods are some of the most successful on-policy methods. They learn the policy directly with a parameterized function, $\pi(a|s;\theta)$. This method is explained further and more explicitly in \ref{paper:weng2018github2}. Instead, we'll focus more on a corner-stone in Policy Gradient methods called \emph{Actor-Critic}. There are a number of algorithms that build off of this algorithm so it is important to understand how it works.

\textbf{Actor-Critic} learns both the value function and the policy using both to influence each other. This is done through the use of an actor and a critic. The actor updates policy parameters in the direction suggested by the critic. The critic updates the value function parameters to make better suggestions for the actor. It can be thought of similar to two siblings playing a video game with the older sibling watching while the younger sibling plays. The older sibling has an understanding of what actions are good and a general idea of what should be done. They influence the actions of the younger sibling with suggestions and recommendations and the younger sibling incorporates those suggestions to their play style. This is more explicitly described in Algorithm \ref{algo:actor_critic}. 

\begin{algorithm}[H]
\label{algo:actor_critic}
\caption{Actor-Critic Algorithm}
\begin{algorithmic}
    \REQUIRE $0 < M \le T$
    \WHILE{$step\_count \le total\_steps$}
        \STATE $\{states, actions, log\_probabilities, rewards\} \leftarrow$ Run policy $\pi_{\theta_{old}}$ in environment for $T$ timesteps
        \STATE compute advantages
        \STATE $step\_count += T$
        \FOR{$epoch = 1,2,...,K$}
            \STATE shuffle $\{state, action, log\_probability, advantage\}$ tuples
            \STATE split into $M$ minibatches
            \FOR{$minibatch = 1,2,...,M$}
                \STATE compute losses
                \STATE $\theta_{old} \leftarrow \theta$
            \ENDFOR
        \ENDFOR
    \ENDWHILE
\end{algorithmic}
\end{algorithm} 

The major challenge still faced, and commonly brought up, in RL is the \textbf{Exploration-Exploitation Dilemma}. \todo{Look into python book for better explanation of this}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Safe Reinforcement Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Safe Reinforcement Learning}
I'll try to groups these papers by the method they use to make the RL "safe". I'll also try to make these summaries more brief.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AlwaysSafe: Reinforcement Learning Without Safety Constraint Violations During Training
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{AlwaysSafe: Reinforcement Learning Without Safety Constraint Violations During Training \cite{Simao2021alwayssafe}}
\textbf{Thiago D. Simão, AAMAS, 2021, \href{https://tdsimao.github.io/publications/Simao2021alwayssafe/}{link}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Safe Exploration in Continuous Action Spaces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Safe Exploration in Continuous Action Spaces \cite{dalal2018safe}}
\textbf{Gal Dalal, arXiv, 2018, \href{https://arxiv.org/abs/1801.08757}{link}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reachability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reachability and Runtime Assurance}
These papers concern the topic of "reachability" and methods for computing reach sets. I'll try to include more of the math involved so I can use it later.

Definitions and explanations of things I understand/know:
\begin{itemize}
    \item Frontier: Essentially the set of all possible $s'$ states
    \item Reachable set: All possible states a system can get to. Usually assumes infinite time and is meant for stability analysis. The set of all frontiers.
    \item Admissible states: a.k.a. "safe sets" but the better term to use. 
    \item Inadmissible sets: "unsafe sets" but doesn't have to be tied to safety, e.g. could be undesirable.
    \item Recoverable states: subset of admissible states. To be recoverable, the safety controller must be able to keep the system within the admissible states.
    \item Flow:
    \item Flow-pipe: 
    \item Reach tube:
    \item Lipschitz continuous function: A function is Lipschitz continuous if and only if there exists $L < \infty$ such that $|f(t, u) - f(t, u^*)| \le L|u - u^*|$ for all $u, u^* \in \mathcal{R}$. This is similar to saying $f'$ is bounded by $L$.
    \item Lipschitz stable: $\dot{x}=f(x(t))$, $x(0)=x_{0}$, where $x(t) \in \mathcal{D} \subseteq \mathcal{R}^{n}$ denotes the system state vector, $\mathcal{D}$ an open set containing the origin, and $f:\mathcal{D} \rightarrow \mathcal{R}^{n}$ continuous on $\mathcal{D}$. Suppose $f$ has an equilibrium at $x_{e}$ so that $f(x_{e})=0$, then this equilibrium is said to be Lyapunov stable, if, for every $\epsilon >0$, there exists a $\delta >0$ such that, if $\|x(0)-x_{e}\|<\delta$, then for every $t\geq 0$ we have $\|x(t)-x_{e}\|<\epsilon$. The equilibrium of the above system is said to be asymptotically stable if it is Lyapunov stable and there exists $\delta >0$ such that, if $\|x(0)-x_{e}\|<\delta$, then $\lim_{t\rightarrow \infty }\|x(t)-x_{e}\|=0$.

\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Safe Reinforcement Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{intro to reachability?}
\textbf{author, conference/journal, year, \href{}{link}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hamilton-Jacobi Reachability: A Brief Overview and Recent Advances
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Hamilton-Jacobi Reachability: A Brief Overview and Recent Advances \cite{bansal2017hamilton}}
\textbf{Somil Bansal, CDC, 2017, \href{https://arxiv.org/abs/1709.07523}{link}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Efficient Reachability Analysis of Closed-Loop Systems with Neural Network Controllers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Efficient Reachability Analysis of Closed-Loop Systems with Neural Network Controllers \cite{everett2021efficient}}
\textbf{Michael Everett, arXiv, 2021, \href{https://arxiv.org/abs/2101.01815}{link}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Verification and Synthesis of Hybrid Systems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Verification and Synthesis of Hybrid Systems \cite{dang2000verification}}
\textbf{Thi Xuan Thao Dang, dissertation, 2000, \href{https://tel.archives-ouvertes.fr/tel-00006738/document}{link}}

In Chapter 5 of this dissertation, the author explains how face lifting works. The initial set of states, which must be represented by an orthogonal polyhedra, is expanded by \emph{lifting} each face according to the defined dynamics. In the initial face lifting algorithm, each face can only move outwards, i.e. the area of the reachable set cannot be smaller than the previous set. The result is an overapproximate reachable set. "However, the goal of ensuring the global error under the desired tolerance is still problematic because of the accumulation of over-approximate error. As a result, there are cases when, in the long run, the over-approximate error becomes too large for the result to be useful." (this is highlighted really well in figure 5.9 and figure 5.11)

To reduce some of the error accumulation from \emph{face lifting}, the author introduces a new method, \emph{mixed face lifting}. In this method, we compute frontiers and the reachable set is a union of the computed frontiers. The frontier includes inward transitions for the faces so a frontier can be smaller than the previous frontier. This reduces the amount of accumulated global error, best shown in figure 5.12. The algorithm for this procedure is shown on page 106 and an aircraft example is explained on page 110.

It will be important to review this material to gain a better understanding of the difference between \emph{frontier} and \emph{reachable set} as that will play an important role in how we determine safety for our aircraft scenario. Note: this method requires ODE's to determine the face transitions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Real-Time Reachability for Verified Simplex Design
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Real-Time Reachability for Verified Simplex Design \cite{johnson2016real}}
\textbf{Taylor T. Johnson, ACM Transactions on Embedded Computing Systems, 2016, \href{https://dl.acm.org/doi/10.1145/2723871}{link}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Real-Time Reachability for Verified Simplex Design
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Real-Time Reachability for Verified Simplex Design \cite{bak2014real}}
\textbf{Stanley Bak, RTSS, 2014, \href{http://stanleybak.com/papers/bak2014rtss.pdf}{link}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Neural Simplex Architecture
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Neural Simplex Architecture \cite{phan2020neural}}
\textbf{Dung T. Phan, NASA Formal Methods Symposium, 2020, \href{https://arxiv.org/abs/1908.00528}{link}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A (Long) Peek into Reinforcement Learning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{TBD}

==> nfm_configurations.tex <==
\subsection{RTA configurations}
In \figref{fig:rta_on}, we show a general method for including RTA in the training loop and purposefully left it vague. In this work, we have separated these various ways of connecting the RTA into the 5 configurations listed and explained below\footnote{More detailed descriptions for the configurations are provided in Appendix \ref{app:configurations}.}. The configurations are listed in order of increasing complexity. Each configuration builds on the previous ones, helping us observe the impact of each addition. %Instead of providing an image showing how each configuration is connected, we show the differences according to what $data$ tuple is collected during training. Because SAC and PPO collect different data tuples during training, we show the most important, shared values recorded in the data tuple.

% \begin{figure}%[htpb]
%     \centering
%     \includegraphics[width=0.4\columnwidth]{figures/rta_config_venn_diagram_5.pdf}
%     \caption{The RTA configurations used in our experiments represented within the three main categories of Safe Reinforcement Learning outlined in Section \ref{sec:SRL}.}
%     \label{fig:rta_configs}
% \end{figure}

% The configurations are explained in detail below. Because SAC and PPO collect different data tuples during training, we must define the configurations using different terms, $data_{SAC}$ and $data_{PPO}$, respectively.


\noindent \textbf{(1) Baseline (no RTA)}

This configuration, demonstrated in \figref{fig:rta_off}, is used as a baseline comparison for all the RTA configurations. In this configuration, the agent is learning using the RL algorithm without any modifications. $\obs$ is the input observation that led to the agent providing the desired action, $\action_{\rm NN}$, and $r$ is the reward value computed by reaching the next state. 
%
%\begin{equation*}
The data tuple is $data = \{\obs, \action_{\rm NN}, r\}$.
%\end{equation*}

\noindent \textbf{(2) Baseline punishment}

In this configuration, we assign a negative reward, i.e. punishment $p<0$, if $unsafe?$ returns true, meaning at least one safety constraint was violated. This configuration adds SRL-style reward shaping to the problem. Instead of only maximizing the reward, the problem has two goals: (1) completing the task and (2) minimizing the punishment, or cost, incurred from violating constraints. In this work. $p$ is constant; however, scaling $p$ according to the severity of the safety violation can be done. The remaining configurations cannot factor in this kind of punishment because they rely on safe exploration which does not allow any violations of the safety constraints.

\begin{equation*}
    data =
    \begin{cases}
    \{\obs, \action_{\rm NN}, r + p\}, & \text{if }unsafe? \\
    \{\obs, \action_{\rm NN}, r\}, & \text{otherwise}
    \end{cases}
\end{equation*}

\noindent \textbf{(3) RTA no punishment}

This configuration is the simplest form of safe exploration. Nothing changes from the baseline configuration except the agent remains safe throughout the training process because of the RTA depicted in \figref{fig:rta_on}.
%\begin{equation*}
    %data =
    %\begin{cases}
The data tuple is $data =\{\obs, \action_{\rm NN}, r\}$, regardless of whether or not the RTA is intervening.%, & \text{if }intervening? \\
    %\{\obs, \action_{\rm NN}, r\}, & \text{otherwise}
    %\end{cases}
%\end{equation*}

\noindent \textbf{(4) RTA punishment}

This configuration adds an element of reward shaping to the previous configuration. Since we want the agent to learn the correct action to take in a scenario without the help of an RTA, we assign a punishment for having the RTA intervene. By adding this punishment, $p$, to the reward, the agent should better identify safe actions.

\begin{equation*}
    data =
    \begin{cases}
    \{\obs, \action_{\rm NN}, r + p\}, & \text{if }intervening? \\
    \{\obs, \action_{\rm NN}, r\}, & \text{otherwise}
    \end{cases}
\end{equation*}

\noindent \textbf{(5) RTA Corrected Action}

In this configuration, we build on the idea of helping the agent identify the correct action to take in states near violating the safety constraints. Instead of punishing the agent for having the RTA intervene, we correct the agent's output to match that of the RTA's. In this manner, the agent only learns the actions actually taken in the environment. 
%
%\\begin{equation*}
The data tuple is $data = \{\obs, \action_{\rm act}, r\}.$
%\end{equation*}

% \todo{Remove NSA since it only work on pendulum. maybe reference it in the future works}
% \noindent \textbf{(6) Neural Simplex Architecture (NSA)}
% This configuration is based on the SRL approach first published in \cite{phan2020neural}. In the authors' original implementation, NSA is used for retraining a learned policy. However, the retraining is done in an online approach, which can be easily adjusted to training a control policy from scratch.

% This configuration includes unsafe experiences while ensuring the agent is always safe during training. The additional data should help the agent develop a much better understanding of the environment and, thus, learn a more optimal policy after fewer timesteps.

% \begin{equation*}
%     data_{SAC} =
%     \begin{cases}
%     \begin{cases}
%     \{\obs, u_{b}, r, \obs'\} \text{ and } \\
%     \{\obs, \action_{\rm NN}, est\_r, est\_\obs'\}
%     \end{cases}, & \text{if }intervening? \\
%     \{\obs, \action_{\rm NN}, r, \obs'\}, & \text{otherwise}
%     \end{cases}
% \end{equation*}

==> nfm_environments.tex <==
\subsection{Training Environments}
We ran our experiments in three environments with varying levels of complexity. Additional information on these environments is provided in Appendix \ref{app:environments}.

% \subsubsection{
\noindent \textbf{Pendulum}

The first environment is a modified version of OpenAI Gym's \emph{Pendulum-v0} environment\footnote{The original Python implementation of this environment can be found at \url{https://github.com/openai/gym/blob/master/gym/envs/classic_control/pendulum.py}}\cite{brockman2016gym}. We chose this environment for its accessibility, simplicity, and previous use in \cite{cheng2019end} as a good indicator of the effectiveness of SRL over standard DRL. We use the same initial conditions and constraints described in their work.

The goal of the agent in this environment is to control an actuator that applies torque to the system to keep a frictionless pendulum upright and within the bounds of $\pm 1rad \approx \pm 46^{\circ}$. Thus, the inequality constraint the RTA is designed to uphold can be written as,
\begin{equation}
\varphi_1(\state) := 1 - |\theta|,  
\end{equation}
where $\theta$ is the displacement angle of the pendulum measured from the upright position. $\theta$ and the angular momentum of the pendulum, $\omega$, are components of the environment state, $\state = [\omega, \theta]$. The observation used as the input for the RL agent is $\obs = [\cos(\theta), \sin(\theta), \omega]$. If this constraint is violated, the episode is terminated.

The RTA design implemented in this environment is a simple implicit simplex design with the backup controller described by Equation \ref{eq:rta_pendulum}.

\begin{equation}
    u_b(\state) = \min\Bigg(\max\Big(\frac{-32}{\pi} \theta, -15\Big), 15\Bigg)
    \label{eq:rta_pendulum}
\end{equation}

The reward function was modified from the original used in \cite{cheng2019end} by adding a constant, $5$, which was chosen in order to make a majority of the reward values positive. By keeping the reward positive, the agent is encouraged to not terminate the episode early. If the reward were mostly negative, the agent might learn that quickly terminating the episode maximizes the return better than remaining near upright. The resulting reward function, Equation \ref{eq:reward_pendulum}, has a cumulative maximum of $1000$ instead of $0$. In the configurations which require a punishment, we use $p=-1$.

\begin{equation}
\label{eq:reward_pendulum}
    r_t = 5 - (\theta_t^2 + 0.1\omega_t^2 + 0.001\action_t^2)
\end{equation}

% \subsubsection{
\noindent \textbf{Spacecraft 2D Spacecraft Docking \& 3D}

The next two environments come from \cite{ravaioli2022safe} and focus on the spacecraft docking problem\footnote{The implementations of these environments can be found at \url{https://github.com/act3-ace/SafeRL}}. In these environments, an active \emph{deputy} spacecraft, under the control of the RL agent, approaches a passive \emph{chief} spacecraft. % in a linearized relative motion reference frame known as Hill's frame \cite{hill1878researches}. The relative motion dynamics between the deputy and chief spacecraft are given by Clohessy-Wiltshire equations \cite{clohessy1960terminal}. 
This scenario is considered in 2D with only the $x$ and $y$ components, as well as 3D with the $x$, $y$, and $z$ components. 
%
The goal of the agent in these environments is to use mounted thrusters that move the \emph{deputy} spacecraft in the $x$, $y$, and $z$ directions to a docking region around the \emph{chief} spacecraft located at the origin. The state and observation are $\state = \obs = [x, y, z, \dot{x}, \dot{y}, \dot{z}]$. If the \emph{chief} spacecraft were moving, the observation might be modified to instead use the relative distances and velocities instead.

RTA is used in these environments to enforce a distance dependent speed limit $\varphi_1(\state)$ and maximum velocity limits $\varphi_2(\state)$-$\varphi_4(\state)$ \cite{dunlap2021Safe, dunlap2021comparing}. %\footnote{More information on how and why these constraints were chosen can be found in \cite{dunlap2021Safe, dunlap2021comparing}.}.
Together, these constraints keep the deputy space craft controllable and prevent collisions caused by the deputy approaching too fast. The distance dependent speed limit is defined as,
\begin{equation} \label{eq:ha1}
    \varphi_1(\state) := \nu_D - \nu_{\rm H} + c d_{\rm H},
\end{equation}
where $\nu_D = 0.2m/s$ defines the maximum allowable docking velocity, $c = 2 s^{-1}$ is a constant, $d_{\rm H} =(x^2+y^2+z^2)^{1/2}$ is the Euclidian distance between the deputy and chief spacecraft, and $\nu_{\rm H} =(\dot{x}^2+\dot{y}^2+\dot{z}^2)^{1/2}$ is the relative speed the deputy is approaching the chief. The maximum velocity, $v_{\rm max} = 10m/s$, limits can be written as inequality constraints,
\begin{equation} \label{eq:ha2}
    \varphi_2(\state) := v_{\rm max}^2 - \dot{x}^2, \quad \varphi_3(\state) := v_{\rm max}^2 - \dot{y}^2, \quad
    \varphi_4(\state) := v_{\rm max}^2 - \dot{z}^2.
\end{equation}

% As described in Section \ref{sec:RTA}, this set of four constraints (excluding $\varphi_4(\state)$ for the 2D scenario) is used to construct the Implicit Simplex and Implicit ASIF RTA filters. By showing that these constraints are control invariant and using the backup control laws from \cite{dunlap2021Safe, dunlap2021comparing}, it is shown that $h_i(\state) = \varphi_i(\state),~i=1,...,4$. This set of control invariant constraints is used to construct the Explicit Simplex and Explicit ASIF RTA filters. 

\begin{table*}[t]
    \centering
    \caption{Spacecraft 2D Spacecraft Docking \& 3D reward function components}
    \begin{tabular}{lc}\hline
        \multicolumn{2}{c}{Terminal Rewards: All Configurations} \\ \hline
        Successfully Docked $(d_{\rm H} \leq 20m$ and $\nu_{\rm H}\leq 0.2 m/s)$ & +1 \\
        Crashed $(d_{\rm H} \leq 20 m$ with a velocity $\nu_{\rm H}> 0.2 m/s)$ & -1 \\
        Out of Bounds $(d_{\rm H} > 200m)$ & -1 \\
        Over Max Time/Control & -1 \\ \hline
        \multicolumn{2}{c}{Dense Reward: All Configurations} \\ \hline
        Proximity & $0.0125(\Delta d_{\rm H} )$ \\ \hline
        \multicolumn{2}{c}{Safety Rewards: Punishment Configurations} \\ \hline
        If RTA is Intervening & $-0.001$  \\
        Over Max Velocity & $-0.1 - 0.1(\nu_{\rm H} - v_{\rm max})$ \\ \hline
    \end{tabular}
    \label{tab:rewards}
\end{table*}

The reward functions for these environments are defined by sparse and dense components defined in \tabref{tab:rewards}\footnote{These values were provided by the authors of the environments during early development and do not match those published in \cite{ravaioli2022safe}. Additionally, these values were chosen with PPO as the target RL algorithm, which helps explain why SAC struggled with learning to complete the task.}. The sparsely defined terminal and safety reward components are only applied if the agent meets the specified requirements. In contrast, the dense reward component is computed after each timestep. In our experiments, the evaluation returns are computed using all the components defined in \tabref{tab:rewards}. However, during training, the safety components are ignored unless the punishment is required by the configuration.

% \subsubsection{Spacecraft 3D Spacecraft Docking}

% \subsubsection{Rejoin?}
